Cooperative Artificial Intelligence

In the future, artificial learning agents are likely to become increasingly widespread in our society. They will interact with both other learning agents and humans in a variety of complex settings including social dilemmas. We argue that there is a need for research on the intersection between game theory and artificial intelligence, with the goal of achieving cooperative artificial intelligence that can navigate social dilemmas well. We consider the problem of how an external agent can promote cooperation between artificial learners by distributing additional rewards and punishments based on observing the actions of the learners. We propose a rule for automatically learning how to create the right incentives by considering the anticipated parameter updates of each agent. Using this learning rule leads to cooperation with high social welfare in matrix games in which the agents would otherwise learn to defect with high probability. We show that the resulting cooperative outcome is stable in certain games even if the planning agent is turned off after a given number of episodes, while other games require ongoing intervention to maintain mutual cooperation. Finally, we reflect on what the goals of multi-agent reinforcement learning should be in the first place, and discuss the necessary building blocks towards the goal of building cooperative AI.

==> Appendices.tex <==
\addcontentsline{toc}{chapter}{Appendices}

% The \appendix command resets the chapter counter, and changes the chapter numbering scheme to capital letters.
%\chapter{Appendices}
\appendix
\chapter{An Appendix About Stuff}
\label{appendixlabel1}
(stuff)

\chapter{Another Appendix About Things}
\label{appendixlabel2}
(things)

\chapter{Colophon}
\label{appendixlabel3}
\textit{This is a description of the tools you used to make your thesis. It helps people make future documents, reminds you, and looks good.}

\textit{(example)} This document was set in the Times Roman typeface using \LaTeX\ and Bib\TeX , composed with a text editor. 
 % description of document, e.g. type faces, TeX used, TeXmaker, packages and things used for figures. Like a computational details section.
% e.g. http://tex.stackexchange.com/questions/63468/what-is-best-way-to-mention-that-a-document-has-been-typeset-with-tex#63503

% Side note:
%http://tex.stackexchange.com/questions/1319/showcase-of-beautiful-typography-done-in-tex-friends

==> New_commands.tex <==
% =============== NEW COMMANDS ===============================================
 \newcommand{\bE}{\mathbb{E}}
 \newcommand{\bR}{\mathbb{R}}
 \newcommand{\cA}{\mathcal{A}}
 \newcommand{\cM}{\mathcal{M}}
 \newcommand{\cS}{\mathcal{S}}
 \newcommand{\cP}{\mathcal{P}}
 \newcommand{\cT}{\mathcal{T}}
 \newcommand{\cO}{\mathcal{O}}
 \newcommand{\cU}{\mathcal{U}}
 \newcommand{\vone}{V_1(\theta_1,\theta_2,s)}
 \newcommand{\vtwo}{V_2(\theta_1,\theta_2,s)}
 \newcommand{\vonen}{V_1(\theta_1,\dots,\theta_N,s)}
 \newcommand{\vtwon}{V_2(\theta_1,\dots,\theta_N,s)}
 \newcommand{\vi}{V_i(\theta_1,\theta_2,s)}
 \newcommand{\vin}{V_i(\theta_1,\dots,\theta_N,s)}
 \newcommand{\vip}{V_i^p(\theta_1,\theta_2,s)}
 \newcommand{\vpn}{V^p(\theta_1,\dots,\theta_N; \theta_p,s)}
 \newcommand{\vinp}{V_i^p(\theta_1,\dots,\theta_N,s)}
 \newcommand{\vitot}{V_i^{\text{tot}}(\theta_1,\theta_2,s)}
 \newcommand{\vintot}{V_i^{\text{tot}}(\theta_1,\dots,\theta_N,s)}
 \newcommand{\vonep}{V_1^p(\theta_1,\theta_2,s)}
 \newcommand{\vtwop}{V_2^p(\theta_1,\theta_2,s)}
 \newcommand{\vt}{V(\theta_1,\theta_2,s)}
 \newcommand{\vtn}{V(\theta_1,\dots,\theta_N,s)}
 \newcommand{\vtnnext}{V(\theta_1+\Delta\theta_1,\dots,\theta_N+\Delta\theta_N,s)}
 \newcommand{\vtp}{V(\theta_1,\theta_2,\theta_p,s)}
 \newcommand{\suminf}{\sum_{t = 0}^{\infty}}
 \newcommand{\sumT}{\sum_{t = 0}^{T}}
 \newcommand{\Rinf}{\suminf\gamma^tr^t}
 \newcommand{\RT}{\sumT\gamma^tr^t}
 \newcommand{\RTi}{\sumT\gamma^tr_i^t}
 \DeclareMathOperator*{\argmax}{arg\,max}
